Monopole Superconductivity in Magnetically Doped Cd$_3$As$_2$

When superconducting pairing occurs between Fermi surfaces with different Chern numbers, the Cooper pairs possess nontrivial pair Berry phase, which enforces pairing gap nodes. The resulting pairing order is further distinguished from the familiar $s$-, $p$-, and $d$-wave pairing orders by a nonzero pair monopole charge and is described by monopole harmonics. To date, this exotic monopole pairing order is yet to be achieved experimentally. We therefore study the magnetically doped Dirac semimetal Cd$_3$As$_2$ as a candidate material for realizing monopole superconductivity with pair monopole charges $q_p=1$ or $2$, depending on the chemical potential. For each case of pair monopole charge, we explore representatives of uniform pairing orders in all allowed irreducible representations of the $C_{4h}$ symmetry of magnetically doped Cd$_3$As$_2$. We demonstrate the distinctions in the monopole analogs of different higher partial wave superconducting orders that result from the combination of topological Fermi surfaces of higher Chern number and crystalline symmetry. In all cases, the patterns of the superconducting phase winding around a Fermi surface are constrained by the topologically invariant total winding number, which depends only on the pair monopole charge and requires nodes in the $q_p\neq 0$ superconducting order. Our work can guide further experimental investigation of monopole orders in the topological semimetal Cd$_3$As$_2$ and can be generalized to other materials with Fermi surfaces of higher Chern number, which enforce monopole pairing order in higher partial waves, such as the monopole analog of $f$-wave pairing.

==> full_table.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Trivial Fermi Pocket}

\todo{Explain table descriptions ($k_\parallel^2 = k_x^2 + k_y^2$)}

\begin{table}[H]
 \begin{tabular}{c||c | c | p{0.25\linewidth} |p{0.2\linewidth}}
  Gap function & Irrep & Matrix Irrep & Phase Winding & Description \\
  \hline \hline
  $\hat{\Delta} = \Delta k_z/k_D (M_{00} - M_{33})$ & $\-^2E_u (\Gamma_3^-)$ & $\-^2E_g (\Gamma_3^+)$&  \vspace{0.2cm}\includegraphics[width=\linewidth]{mu0035/g00m33.pdf} & $k_{\parallel}^2 e^{2i\phi}$ nodes on $k_z$ axis.
  \\
  
  \hline
  $\hat{\Delta} = \Delta k_z/k_D (M_{00} + M_{33})$ & $\-^1E_u (\Gamma_4^-)$ & $\-^1E_g (\Gamma_4^+)$ & \vspace{0.2cm}\includegraphics[width=\linewidth]{mu0035/g00p33.pdf} & Gap function only vanishes at $k_z = 0$.
  \\
  
  \hline
  $\hat{\Delta} = \Delta k_z/k_D M_{13}$ & $A_u (\Gamma_1^-)$ & $A_g (\Gamma_1^+)$ &  \vspace{0.2cm}\includegraphics[width=\linewidth]{mu0035/g13.pdf} & $k_{\parallel}^3 e^{-i\phi}$ nodes on $k_z$ axis.
  \\
  
  \hline
  $\hat{\Delta} = \Delta M_{02}$ & $B_u (\Gamma_2^-)$ & $B_u (\Gamma_2^-)$ & \vspace{0.2cm}\includegraphics[width=\linewidth]{mu0035/g02.pdf} & $k_{\parallel} e^{i\phi}$ nodes on $k_z$ axis.
  \\
 \end{tabular}
 \caption{Table of representative phase winding behavior on the smaller $C=0$ Fermi pocket at $\mu = 0.035eV$.}
 \label{tab:mu0035}
\end{table}



\begin{table}[H]
 \begin{tabular}{c||c | c | p{0.25\linewidth} |p{0.2\linewidth}}
  Gap function & Irrep & Matrix Irrep & Phase Winding & Description \\
  \hline \hline
  
  $\hat{\Delta} = \Delta k_z/k_D (M_{03} + M_{30})$ & $\-^1E_u (\Gamma_4^-)$ & $\-^1E_g (\Gamma_4^+)$ &  \vspace{0.2cm}\includegraphics[width=\linewidth]{mu0035/g03p30.pdf} & Gap function only vanishes at $k_z = 0$.
  \\
  \hline
  
  $\hat{\Delta} = \Delta k_z/k_D (M_{03} - M_{30})$ & $\-^2E_u (\Gamma_3^-)$ & $\-^2E_g (\Gamma_3^+)$ &  \vspace{0.2cm}\includegraphics[width=\linewidth]{mu0035/g03m30.pdf} & $k_\parallel^2 e^{2i\phi}$ nodes on $k_z$ axis.
  \\
  \hline
  
  $\hat{\Delta} = \Delta (M_{12} + M_{21})$ & $\-^2E_u (\Gamma_3^-)$ & $\-^2E_u (\Gamma_3^-)$ &  \vspace{0.2cm}\includegraphics[width=\linewidth]{mu0035/g12p21.pdf} & $k_\parallel^2 e^{2i\phi}$ nodes on $k_z$ axis.
  \\
  \hline
  
  $\hat{\Delta} = \Delta (M_{12} - M_{21})$ & $\-^1E_u (\Gamma_4^-)$ & $\-^1E_u (\Gamma_4^-)$ &  \vspace{0.2cm}\includegraphics[width=\linewidth]{mu0035/g12m21.pdf} & $k_\parallel^4$ nodes on $k_z$ axis.
  \\
  \hline
  
  $\hat{\Delta} = \Delta M_{32}$ & $B_u (\Gamma_2^-)$ & $B_u (\Gamma_2^-)$ &  \vspace{0.2cm}\includegraphics[width=\linewidth]{mu0035/g32.pdf} & $k_\parallel e^{i\phi}$ nodes on $k_z$ axis.
  \\
  \hline
 \end{tabular}
 \caption{Table of phase winding behavior on the smaller $C=0$ Fermi pocket at $\mu = 0.035eV$.}
 \label{tab:mu0035rest}
\end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{$C=1$ Fermi Pocket}

\begin{table}[H]
 \begin{tabular}{c||c | c | p{0.25\linewidth}| p{0.25\linewidth} |p{0.1\linewidth}}
  Gap function & Irrep & Matrix Irrep & Phase Winding North & Phase Winding South & Description \\
  \hline \hline
  
   $\hat{\Delta} = \Delta k_z/k_D (M_{00} - M_{33})$ & $\-^2E_u (\Gamma_3^-)$ & $\-^2E_g (\Gamma_3^+)$&  \vspace{0.2cm}\includegraphics[width=\linewidth]{mu002/North/g00m33.pdf} & \vspace{0.2cm}\includegraphics[width=\linewidth]{mu002/South/g00m33.pdf}&  $k_{\parallel}^2 e^{2i\phi}$ gap function node at $N$, gapped at $S$.
  \\
  
  \hline
  $\hat{\Delta} = \Delta k_z/k_D (M_{00} + M_{33})$ & $\-^1E_u (\Gamma_4^-)$ & $\-^1E_g (\Gamma_4^+)$ & \vspace{0.2cm}\includegraphics[width=\linewidth]{mu002/North/g00p33.pdf} & \vspace{0.2cm}\includegraphics[width=\linewidth]{mu002/South/g00p33.pdf} & Gapped at $N$, $k_{\parallel}^2 e^{-2i\phi}$ gap function node at $S$.
  \\
  
  \hline
  $\hat{\Delta} = \Delta k_z/k_D M_{13}$ & $A_u (\Gamma_1^-)$ & $A_g (\Gamma_1^+)$ &  \vspace{0.2cm}\includegraphics[width=\linewidth]{mu002/North/g13.pdf} & \vspace{0.2cm}\includegraphics[width=\linewidth]{mu002/South/g13.pdf} 
  & $k_{\parallel}^3 e^{-i\phi}$ gap function node at $N$, $k_{\parallel}^3 e^{-3i\phi}$ gap function node at $S$.
  \\
  
  
  \hline
  $\hat{\Delta} = \Delta M_{02}$ & $B_u (\Gamma_2^-)$ & $B_u (\Gamma_2^-)$ & \vspace{0.2cm}\includegraphics[width=\linewidth]{mu002/North/g02.pdf} & \vspace{0.2cm}\includegraphics[width=\linewidth]{mu002/South/g02.pdf} 
  & $k_{\parallel} e^{i\phi}$ gap function node at $N$, $k_{\parallel} e^{-i\phi}$ gap function node at $S$.
  \\
  
 \end{tabular}
 \caption{Table of representative phase winding behavior for the $C=1$ pocket at $\mu = 0.02eV$.}
 \label{tab:mu002}
\end{table}

\begin{table}[H]
 \begin{tabular}{c||c | c | p{0.25\linewidth}| p{0.25\linewidth} |p{0.1\linewidth}}
  Gap function & Irrep & Matrix Irrep & Phase Winding North & Phase Winding South & Description \\
  \hline \hline
  
     $\hat{\Delta} = \Delta k_z/k_D (M_{03} + M_{30})$ & $\-^1E_u (\Gamma_4^-)$ & $\-^1E_g (\Gamma_4^+)$ &  \vspace{0.2cm}\includegraphics[width=\linewidth]{mu002/North/g03p30.pdf} & \vspace{0.2cm}\includegraphics[width=\linewidth]{mu002/South/g03p30.pdf}& Gapped at $N$, $k_\parallel^2 e^{-2i\phi}$ gap function node at $S$.
     
     \\
     \hline
    $\hat{\Delta} = \Delta k_z/k_D (M_{03} - M_{30})$ & $\-^2E_u (\Gamma_3^-)$ & $\-^2E_g (\Gamma_3^+)$ &  \vspace{0.2cm}\includegraphics[width=\linewidth]{mu002/North/g03m30.pdf} & \vspace{0.2cm}\includegraphics[width=\linewidth]{mu002/South/g03m30.pdf}& $k_\parallel e^{2i\phi}$ gap function node at $N$, gapped at $S$.
    
    \\
    \hline
    $\hat{\Delta} = \Delta (M_{12} + M_{21})$ & $\-^2E_u (\Gamma_3^-)$ & $\-^2E_u (\Gamma_3^-)$ &  \vspace{0.2cm}\includegraphics[width=\linewidth]{mu002/North/g12p21.pdf} & \vspace{0.2cm}\includegraphics[width=\linewidth]{mu002/South/g12p21.pdf} & $k_\parallel^2 e^{-2i\phi}$ gap function node at $N$, $k_\parallel^4 e^{-4i\phi}$ gap function node at $S$.
    
    \\
    \hline
    $\hat{\Delta} = \Delta (M_{12} - M_{21})$ & $\-^1E_u (\Gamma_4^-)$ & $\-^1E_u (\Gamma_4^-)$ &  \vspace{0.2cm}\includegraphics[width=\linewidth]{mu002/North/g12m21.pdf} & \vspace{0.2cm}\includegraphics[width=\linewidth]{mu002/South/g12m21.pdf} & $k_\parallel^4$ gap function node at $N$, $k_\parallel^2 e^{-2i\phi}$ gap function node at $S$.
    
    \\
    \hline
    $\hat{\Delta} = \Delta M_{32}$ & $B_u (\Gamma_2^-)$ & $B_u (\Gamma_2^-)$ &  \vspace{0.2cm}\includegraphics[width=\linewidth]{mu002/North/g32.pdf} & \vspace{0.2cm}\includegraphics[width=\linewidth]{mu002/South/g32.pdf} & $k_\parallel e^{i\phi}$ gap function node at $N$, $k_\parallel e^{-i\phi}$ gap function node at $S$.
  \\
  
  \end{tabular}
   \caption{Table of phase winding behavior for the $C=1$ hole pocket at $\mu = 0.02 eV$.}
   \label{tab:mu002rest}
\end{table}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{$C=2$ Fermi Pocket}

\begin{table}[H]
 \begin{tabular}{c||c | c | p{0.25\linewidth}| p{0.25\linewidth} |p{0.1\linewidth}}
  Gap function & Irrep & Matrix Irrep & Phase Winding North & Phase Winding South & Description \\
  \hline \hline
  
   $\hat{\Delta} = \Delta k_z/k_D (M_{00} - M_{33})$ & $\-^2E_u (\Gamma_3^-)$ & $\-^2E_g (\Gamma_3^+)$&  \vspace{0.2cm}\includegraphics[width=\linewidth]{mu0/North/g00m33.pdf} & \vspace{0.2cm}\includegraphics[width=\linewidth]{mu0/South/g00m33.pdf}& Gapped at N and S. Four nodes with $e^{i \phi'}$ local winding at $\phi = 0, \pm \pi/2, \pi$ around concave region near S.
  \\
  
  \hline
  $\hat{\Delta} = \Delta k_z/k_D (M_{00} + M_{33})$ & $\-^1E_u (\Gamma_4^-)$ & $\-^1E_g (\Gamma_4^+)$ & \vspace{0.2cm}\includegraphics[width=\linewidth]{mu0/North/g00p33.pdf} & \vspace{0.2cm}\includegraphics[width=\linewidth]{mu0/South/g00p33.pdf} & $k_\parallel^2 e^{-2i\phi}$ nodes at N and S poles. Four nodes with $e^{i \phi'}$ local winding at $\phi = 0, \pm \pi/2, \pi$ around concave region near S.
  \\
  
  \hline
  $\hat{\Delta} = \Delta k_z/k_D M_{13}$ & $A_u (\Gamma_1^-)$ & $A_g (\Gamma_1^+)$ &  \vspace{0.2cm}\includegraphics[width=\linewidth]{mu0/North/g13.pdf} & \vspace{0.2cm}\includegraphics[width=\linewidth]{mu0/South/g13.pdf} 
  & 
  $k_{\parallel}^3 e^{-3i\phi}$ gap function node at $N$, $k_{\parallel}^3 e^{i\phi}$ gap function node at $S$.
  \\
  
  
  \hline
  $\hat{\Delta} = \Delta M_{02}$ & $B_u (\Gamma_2^-)$ & $B_u (\Gamma_2^-)$ & \vspace{0.2cm}\includegraphics[width=\linewidth]{mu0/North/g02.pdf} & \vspace{0.2cm}\includegraphics[width=\linewidth]{mu0/South/g02.pdf} 
  & $k_\parallel e^{-i\phi}$ nodes at N and S poles. Four nodes with $e^{i \phi'}$ local winding at $\phi = \pm \pi/4, \pm 3\pi/4$ around concave region near S.
  \\
  
 \end{tabular}
 \caption{Table of representative phase winding behavior for the $C=2$ hole pocket at $\mu = 0 eV$.}
 \label{tab:mu0}
\end{table}

\begin{table}[H]
 \begin{tabular}{c||c | c | p{0.25\linewidth}| p{0.25\linewidth} |p{0.1\linewidth}}
  Gap function & Irrep & Matrix Irrep & Phase Winding North & Phase Winding South & Description \\
  \hline \hline
  
     $\hat{\Delta} = \Delta k_z/k_D (M_{03} + M_{30})$ & $\-^1E_u (\Gamma_4^-)$ & $\-^1E_g (\Gamma_4^+)$ &  \vspace{0.2cm}\includegraphics[width=\linewidth]{mu0/North/g03p30.pdf} & \vspace{0.2cm}\includegraphics[width=\linewidth]{mu0/South/g03p30.pdf}& $k_\parallel^2 e^{-2i\phi}$ nodes at $N$ and $S$ poles. Four nodes with $e^{i\phi'}$ local winding at $\phi = \pm \pi/4, \pm 3\pi/4$ around concave region near $S$.
     
     \\
     \hline
    $\hat{\Delta} = \Delta k_z/k_D (M_{03} - M_{30})$ & $\-^2E_u (\Gamma_3^-)$ & $\-^2E_g (\Gamma_3^+)$ &  \vspace{0.2cm}\includegraphics[width=\linewidth]{mu0/North/g03m30.pdf} & \vspace{0.2cm}\includegraphics[width=\linewidth]{mu0/South/g03m30.pdf}& Gapped at N and S. Four nodes with $e^{i \phi'}$ local winding at $\phi = \pm \pi/4, \pm 3\pi/4$ around concave region near S.
    
    \\
    \hline
    $\hat{\Delta} = \Delta (M_{12} + M_{21})$ & $\-^2E_u (\Gamma_3^-)$ & $\-^2E_u (\Gamma_3^-)$ &  \vspace{0.2cm}\includegraphics[width=\linewidth]{mu0/North/g12p21.pdf} & \vspace{0.2cm}\includegraphics[width=\linewidth]{mu0/South/g12p21.pdf} & $k_\parallel^4 e^{-4i\phi}$ gap function node at $N$, $k_\parallel^4$ gap function node at $S$.
    
    \\
    \hline
    $\hat{\Delta} = \Delta (M_{12} - M_{21})$ & $\-^1E_u (\Gamma_4^-)$ & $\-^1E_u (\Gamma_4^-)$ &  \vspace{0.2cm}\includegraphics[width=\linewidth]{mu0/North/g12m21.pdf} & \vspace{0.2cm}\includegraphics[width=\linewidth]{mu0/South/g12m21.pdf} & $k_\parallel^2 e^{-2i\phi}$ gap function node at $N$, $k_\parallel^2 e^{2i\phi}$ gap function node at $S$.
    
    \\
    \hline
    $\hat{\Delta} = \Delta M_{32}$ & $B_u (\Gamma_2^-)$ & $B_u (\Gamma_2^-)$ &  \vspace{0.2cm}\includegraphics[width=\linewidth]{mu0/North/g32.pdf} & \vspace{0.2cm}\includegraphics[width=\linewidth]{mu0/South/g32.pdf} & $k_\parallel e^{-i\phi}$ gap function nodes at $N$ and $S$ poles. Four nodes with $e^{i\phi'}$  local winding at $\phi = 0, \pm \pi/2, \pi$ around concave region near $S$.
  \\
  
  \end{tabular}
   \caption{Table of phase winding behavior for the $C=2$ hole pocket at $\mu = 0 eV$.}
   \label{tab:mu0rest}
\end{table}
